Dual Skipping Guidance for Document Retrieval with Learned Sparse Representations

This paper proposes a dual skipping guidance scheme with hybrid scoring to accelerate document retrieval that uses learned sparse representations while still delivering a good relevance. This scheme uses both lexical BM25 and learned neural term weights to bound and compose the rank score of a candidate document separately for skipping and final ranking, and maintains two top-k thresholds during inverted index traversal. This paper evaluates time efficiency and ranking relevance of the proposed scheme in searching MS MARCO TREC datasets.

==> table/deepimpact-passage.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{DeepImpact-Passage (Intel NUC).\label{tab:p-di}}
    \begin{tabular}{c|ccc|c}
    \hline \hline
     Methods & NDCG & MRR & MAP & Time \\ \hline
     BM25 & 0.2965 & 0.1835 & 0.1805 & 17 \\
     DI & 0.4557 & 0.3392 & 0.3340 & 71 \\
     DI (BM25 guided) & 0.4556 & 0.3391 & 0.3339 & 57 \\
     DI (BM25 + DI guided) & 0.4236 & 0.3252 & 0.3201 & 46 \\
     DI (Index sep, BM25 guided) & & 0.3345 & & 38 \\
     DI (Index sep, BM25 + DI guided) & & 0.3235 & & 35 \\
     BM25 then DI (BM25 guided) & 0.4527 & 0.3385 & 0.3332 & 17+30 \\
     BM25 then DI (BM25 + DI guided) &  & 0.3246 & & 17+24 \\
     \hline \hline
    \end{tabular}
\end{table*}

==> table/unicoil-alpha.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage Dev Alpha Experiment.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Trec19 Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline

     Unicoil (B$_{T5}$), 0 & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 35 & 78 &  &  &  \\
     Unicoil (B$_{T5}$), 0.00005 (10\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 31 & 34 & 76 &  &  &  \\
     Unicoil (B$_{T5}$), 0.0001 (20\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 34 & 37 & 80 &  &  &  \\
     Unicoil (B$_{T5}$), 0.0004 (50\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 35 & 40 & 84 &  &  &  \\
     Unicoil (B$_{T5}$), 0.004 (90\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 41 & 47 & 111 &  &  &  \\
    
     \hline
     Unicoil (B$_{T5}$+L), 0 & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 34 & 77 &  &  &  \\
      Unicoil (B$_{T5}$+L), 0.00005 (10\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 30 & 32 & 73 &  &  &  \\
     Unicoil (B$_{T5}$+L), 0.0001 (20\%) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 34 & 37 & 79 &  &  &  \\
     Unicoil (B$_{T5}$+L), 0.0004 (50\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 35 & 40 & 84 &  &  &  \\
     Unicoil (B$_{T5}$+L), 0.004 (90\%) & 2.0G & 0.4735 & 0.3577 & 0.9527 & 40 & 47 & 111 &  &  &  \\
    %  Unicoil (SepInd, B) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 106 & 115 & 253 &  &  &  \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 105 & 115 & 250 &  &  &  \\ 
    \hline
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}

==> table/unicoil-document.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Document.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 6.4G & 0.3389 & 0.2173 & 0.8651 & 149 & 167 & 355 & & & \\
     BM25+ & & & & & & & \\
     Unicoil & 6.9G & 0.4736 & 0.3535 & 0.9426 & 336 & 497 & 1456 & & & \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 10.3G & 0.4735 & 0.3536 & 0.9403 & 193 & 212 & 454 & & & \\
     Unicoil (B+L) & 10.3G & 0.4735 & 0.3536 & 0.9403 & 189 & 208 & 444 & & & \\
    %  Unicoil (SepInd, B) & 13.3G & & & & & & & & & \\
    %  Unicoil (SepInd, B+L) & 13.3G  & 0.4415 & 0.3239 & 0.9287 & 236 & 268 & 603 & & & \\
    %  Unicoil (B Known thres) & 16.7G & 0.4735 & 0.3536 & 0.3536 & 191 & 211 & 455 & & & \\
    %  Unicoil (SepInd, B Known thres) & & & & & & & & & & \\
     \hline \hline
    \end{tabular}
\end{table*}


% \begin{table*}[tpbh]
%     \centering
%         \caption{Unicoil-Document (Expanse).\label{tab:d-uni}}
%     \begin{tabular}{c|ccc|c}
%     \hline \hline
%      Methods & NDCG & MRR & MAP & Time \\ \hline
%      BM25 & 0.3469 & 0.2263 & 0.2263 & 222 \\
%      Unicoil & 0.4736 & 0.3535 & 0.3535 & 552 \\
%      Unicoil (BM25 guided) & 0.4735 & 0.3536 & 0.3536 & 290 \\
%      \hline \hline
%     \end{tabular}
% \end{table*}

==> table/unicoil-passage.tex <==
\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage Dev.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Dev Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 0.9G & 0.2972 & 0.1837 & 0.8374 & 16 & 19 & 46 & 14 & 17 & 42 \\
     BM25+0 & 1.4G & 0.2972 & 0.1837 & 0.8374 & 42 & 44 & 92 & & & \\
     BM25-T5 & 1.4G & 0.3954 & 0.2709 & 0.9363 & 33 & 35 & 74 &  &  &  \\ \hline
     Unicoil & 1.4G & 0.4735 & 0.3577 & 0.9527 & 44 & 52 & 135 & 43 & 50 & 132 \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 40 & 44 & 95 & 40 & 43 & 92 \\
     Unicoil (B$_{T5}$) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 35 & 78 &  &  &  \\
     Unicoil (B+L) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 38 & 42 & 88 & 38 & 41 & 88 \\
     Unicoil (B$_{T5}$+L) & 2.0G & 0.4732 & 0.3576 & 0.9542 & 32 & 34 & 77   &  &  &  \\ 
     Unicoil (DSHS) & 2.0G & 0.4754 & 0.3605 & 0.9530 & 30 & 33 & 76 &  &  &  \\ \hline
    %  Unicoil (SepInd, B) & 2.1G & 0.4547 & 0.3389 & 0.9348 & 34 & 38 & 86 & 34 & 37 & 85 \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.4547 & 0.3389 & 0.9348 & 31 & 35 & 77 & 31 & 34 & 75 \\ \hline
     DeepImpact & 1.5G & 0.4557 & 0.3392 &  &  & 71 &  & & & \\
    %  DeepImpact- & & & & & & & & & & \\
     DeepImpact (B) & 2.2G & 0.4556 & 0.3391 &  & & 57 & & & & \\
     DeepImpact (B+L) & 2.2G & 0.4236 & 0.3252 &  & & 46 & & & & \\
    %  DeepImpact (SepInd, B) & 2.1G & & & & & & & & & \\
    %  DeepImpact (SepInd, B+L) & 2.1G & & 0.3235 &  & & 35 & & & & \\ 
    \hline
     SpladesV2 & 4.5G & 0.4618 & 0.3417 & 0.9613 & 49 & 60 & 151 & & & \\
    %  SpladesV2- & & & & & & & & & & \\
     SpladeV2 (B) & 6.7G & 0.4617 & 0.3417 & 0.9608 & 49 & 58 & 133 & & & \\
     SpladeV2 (B$_{T5}$) & 6.7G & 0.4613 & 0.3417 & 0.9581 & 43 & 50 & 108 & & & \\
     SpladeV2 (B+L) & 6.7G & 0.4617 & 0.3417 & 0.9608 & 48 & 57 & 130 & & & \\
     SpladeV2 (B$_{T5}$+L) & 6.7G & 0.4614 & 0.3417 & 0.9584 & 41 & 48 & 107 & & & \\
     SpladeV2 (DSHS) & 6.7G & 0.4623 & 0.3424 & 0.9589 & 42 & 49 & 110 & & & \\
    %  SpladeV2 (SepInd, B) & 2.1G & & & & & & & & & \\
    %  SpladeV2 (SepInd, B+L) & 2.1G & &  &  & & & & & & \\ \hline
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}

\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage TREC19.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Trec19 Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 0.9G & 0.5501 & 0.7396 & 0.7081 & 54 & 63 & 144 & 53 & 52 & 140 \\
    %  BM25+0 & 1.4G & 0.6653 & 0.8857 & 0.7586 & 102 & 109 & 243 &  &  &  \\
     BM25-T5 & 1.4G & 0.6653 & 0.8857 & 0.7586 & 77 & 78 & 169 &  &  &  \\ \hline
     Unicoil & 1.4G & 0.7163 & 0.9767 & 0.7822 & 148 & 230 & 722 & 135 & 229 & 720 \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 2.0G & 0.7171 & 0.9767 & 0.7839 & 112 & 113 & 233 & 112 & 113 & 230 \\
     Unicoil (B$_{T5}$) & 2.0G & 0.7171 & 0.9767 & 0.7839 & 91 & 89 & 197 &  &  &  \\
     Unicoil (B+L) & 2.0G & 0.7169 & 0.9767 & 0.7836 & 109 & 108 & 222 & 107 & 107 & 221 \\
     Unicoil (B$_{T5}$+L) & 2.0G & 0.7169 & 0.9767 & 0.7836 & 86 & 84 & 172 &  &  &  \\
     Unicoil (DSHS) & 2.0G & 0.7194 & 0.9767 & 0.7854 & 86 & 84 & 170 & 85 & 83 & 169 \\
    %  Unicoil (SepInd, B) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 106 & 115 & 253 &  &  &  \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 105 & 115 & 250 &  &  &  \\ 
    \hline
    
    DeepImpact & 1.5G & 0. & 0. & 0. &  &  &  &  &  &  \\
    DeepImpact (B) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     
     \hline
     
     SpladeV2 & 4.5G & 0.7346 & 0.9612 & 0.8214 & 119 & 159 & 416 &  &  &  \\
    SpladeV2 (B) & 6.7G & 0.7346 & 0.9612 & 0.8217 & 85 & 112 & 260 &  &  &  \\
     SpladeV2 (B$_{T5}$) & 6.7G & 0.7354 & 0.9612 & 0.8245 & 90 & 109 & 249 &  &  &  \\
     SpladeV2 (B+L) & 6.7G & 0.7343 & 0.9612 & 0.8213 & 82 & 107 & 249 &  &  &  \\
     SpladeV2 (B$_{T5}$+L) & 6.7G & 0.7354 & 0.9612 & 0.8244 & 72 & 89 & 201 &  &  &  \\
     SpladeV2 (DSHS) & 6.7G & 0.7379 & 0.9612 & 0.8256 & 71 & 88 & 200 &  &  &  \\
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}

\begin{table*}[tpbh]
    \centering
        \caption{Unicoil-Passage TREC20.\label{tab:p-uni}}
    \begin{tabular}{c|c|ccc|ccc|ccc}
    \hline \hline
    & & \multicolumn{3}{c|}{Trec20 Metrics} &\multicolumn{3}{c|}{BMW Time}& \multicolumn{3}{c}{vBMW Time} \\
     Methods & Storage & NDCG & MRR & Recall & Median & Mean & 95th perc. & Median & Mean & 95th perc. \\ \hline
     BM25 & 0.9G & 0.5156 & 0.8286 & 0.6455 & 47 & 56 & 161 & 43 & 54 & 157 \\
    %  BM25+0 & 1.4G & 0. & 0. & 0. &  &  &  &  &  &  \\
     BM25-T5 & 1.4G & 0.6531 & 0.9444 & 0.7564 & 67 & 75 & 183 &  &  &  \\ \hline
     Unicoil & 1.4G & 0.6937 & 0.9338 & 0.7758 & 142 & 247 & 896 & 136 & 240 & 895 \\
    %  Unicoil- & & & & & & & & & & \\
     Unicoil (B) & 2.0G & 0.6940 & 0.9338 & 0.7765 & 93 & 105 & 273 & 95 & 108 & 251 \\
     Unicoil (B$_{T5}$) & 2.0G & 0.6932 & 0.9338 & 0.7732 & 74 & 80 & 202 &  &  &  \\
     Unicoil (B+L) & 2.0G & 0.6940 & 0.9338 & 0.7765 & 88 & 100 & 243 & 86 & 98 & 240 \\
     Unicoil (B$_{T5}$+L) & 2.0G & 0.6930 & 0.9338 & 0.7729 & 74 & 79 & 200 &  &  &  \\
     Unicoil (DSHS) & 2.0G & 0.6972 & 0.9369 & 0.7760 & 74 & 78 & 198 &  &  &  \\
    %  Unicoil (SepInd, B) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 106 & 115 & 253 &  &  &  \\
    %  Unicoil (SepInd, B+L) & 2.1G & 0.6388 & 0.9360 & 0.7022 & 105 & 115 & 250 &  &  &  \\ 
    \hline
    
    DeepImpact & 1.5G & 0. & 0. & 0. &  &  &  &  &  &  \\
    DeepImpact (B) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     DeepImpact (B$_{T5}$+L) & 2.2G & 0. & 0. & 0. &  &  &  &  &  &  \\
     
     \hline
     
     SpladeV2 & 4.5G & 0.7068 & 0.9374 & 0.7969 & 105 & 155 & 464 &  &  &  \\
    SpladeV2 (B) & 6.7G & 0.7042 & 0.9374 & 0.7922 & 80 & 108 & 320 &  &  &  \\
     SpladeV2 (B$_{T5}$) & 6.7G & 0.7049 & 0.9374 & 0.7955 & 82 & 107 & 297 &  &  &  \\
     SpladeV2 (B+L) & 6.7G & 0.7042 & 0.9374 & 0.7922 & 77 & 104 & 315 &  &  &  \\
     SpladeV2 (B$_{T5}$+L) & 6.7G & 0.7050 & 0.9374 & 0.7957 & 65 & 86 & 245 &  &  &  \\
     SpladeV2 (DSHS) & 6.7G & 0.7065 & 0.9374 & 0.7982 & 66 & 86 & 245 &  &  & \\
     
    %  Unicoil (B Known thres) & 2.9G & 0.4732 & 0.3576 & 0.3524 & 37 & 42 & 92 \\
    %  Unicoil (SepInd, B Known thres) & & & & & 34 & 41 & 92 \\
     \hline \hline
    \end{tabular}
\end{table*}
